Is Best-of-N the Best of Them? Coverage, Scaling, and Optimality in Inference-Time Alignment

Inference-time computation offers a powerful axis for scaling the performance of language models. However, naively increasing computation in techniques like Best-of-N sampling can lead to performance degradation due to reward hacking. Toward a theoretical understanding of how to best leverage additional computation, we focus on inference-time alignment, which we formalize as the problem of improving the quality of responses drawn from a pre-trained policy, given a prompt of interest and access to an imperfect reward model. We analyze the performance of inference-time alignment algorithms in terms of (i) response quality, and (ii) compute, and provide new results that highlight the importance of the pre-trained policy's coverage over high-quality responses for performance and compute scaling: 1. We show that Best-of-$N$ alignment with an ideal choice for $N$ can achieve optimal performance under stringent notions of coverage, but provably suffers from reward hacking when $N$ is large, and fails to achieve tight guarantees under more realistic coverage conditions. 2. We introduce $\texttt{InferenceTimePessimism}$, a new algorithm which mitigates reward hacking through deliberate use of inference-time compute, implementing the principle of pessimism in the face of uncertainty via rejection sampling; we prove that its performance is optimal and does not degrade with $N$, meaning it is scaling-monotonic. We complement our theoretical results with an experimental evaluation that demonstrate the benefits of $\texttt{InferenceTimePessimism}$ across a variety of tasks and models.

==> old_macros.tex <==


\newcommand{\mainalg}{\texttt{InferenceTimePessimism}\xspace}
\newcommand{\mainalglong}{Inference-Time Pessimism\xspace}

\newcommand{\bonalg}{\texttt{BoN}\xspace}
\newcommand{\bonalglong}{Best-of-N Alignment\xspace}

\newcommand{\densobs}{expert densities\xspace}
\newcommand{\DensObs}{Expert Densities\xspace}

\newcommand{\Capx}{C_{\texttt{apx}}}

\newcommand{\vepsstatn}{\vepsstat(n)}
\newcommand{\vepsstatsn}{\vepsstat^2(n)}

\newcommand{\vepsmis}{\veps_{\texttt{mis}}}


\newcommand{\dirac}{\updelta}

\newcommand{\pia}{\pi^{\afrak}}
\newcommand{\pib}{\pi^{\bfrak}}
\newcommand{\Llayer}{L_{\texttt{layer}}}
\newcommand{\piref}{\pi^{\texttt{ref}}}

\newcommand{\Shat}{\wh{S}}

\newcommand{\Astar}{A^{\pistar}}

\newcommand{\sigmab}{\wb{\sigma}}
\newcommand{\sigmabs}{\wb{\sigma}_{\pistar}}

\newcommand{\Hstar}{H^{\star}}%
\newcommand{\pitil}{\wt{\pi}}%

\newcommand{\Jhat}{\wh{J}}


\newcommand{\gbar}{\wb{g}}

\newcommand{\mutil}{\wt{\mu}}

\newcommand{\sigmastar}{\sigma_{\pistar}}

\newcommand{\Lmax}{L_{\texttt{max}}}
\newcommand{\Lmaxhat}{\wh{L}_{\texttt{max}}}
\newcommand{\vepsapx}{\veps_{\texttt{apx}}}
\newcommand{\vepsopt}{\veps_{\texttt{opt}}}

\newcommand{\Drho}[2]{\rho\prn*{#1\dmid{}#2}}

\newcommand{\murec}{\mu}

\newcommand{\astart}[1][t]{a^{\star,\sss{#1}}}
\newcommand{\astari}[1][i]{a^{\star,\sss{#1}}}
\newcommand{\vepsapxh}{\veps_{\texttt{apx},h}}

\newcommand{\Qstar}{Q^{\pistar}}
\newcommand{\Vstar}{V^{\pistar}}


  \newcommand{\Lbc}{L_{\textsf{bc}}}
    \newcommand{\Lhatbc}{\wh{L}_{\textsf{bc}}}

\newcommand{\traj}{o}

\renewcommand{\dagger}{\texttt{Dagger}\xspace}
\newcommand{\aggrevate}{\texttt{Aggrevate}\xspace}
\newcommand{\loglossbc}{\texttt{LogLossBC}\xspace}
\newcommand{\loglossdagger}{\texttt{LogLossDagger}\xspace}

\newcommand{\Unif}{\mathsf{Unif}}

\newcommand{\phistar}{\phi^{\star}}
\newcommand{\gstar}{g^{\star}}

\newcommand{\phidel}{\phi^\triangle}
\newcommand{\MU}{\mathcal{U}}
\newcommand{\bfi}{\mathbf{i}}



\newcommand{\pibar}{\wb{\pi}}

\newcommand{\Cpush}{C_{\mathsf{push}}}

  \newcommand{\sfrak}{\mathfrak{s}}
  \newcommand{\afrak}{\mathfrak{a}}
  \newcommand{\bfrak}{\mathfrak{b}}
  \newcommand{\cfrak}{\mathfrak{c}}
  \newcommand{\xfrak}{\mathfrak{x}}
  \newcommand{\yfrak}{\mathfrak{y}}
  \newcommand{\zfrak}{\mathfrak{z}}
    \newcommand{\bxi}{\mb{\xi}}
  \newcommand{\bs}{\mathbf{s}}
  \newcommand{\ba}{\mathbf{a}}
  \newcommand{\bx}{\mathbf{x}}
  \newcommand{\br}{\mathbf{r}}


\newcommand{\vepsstat}{\veps_{\texttt{stat}}}

\newcommand{\ppr}{p_{\mathrm{pr}}}
\newcommand{\ppo}{p_{\mathrm{po}}}

\newcommand{\gammastar}{\gamma^{\star}}

\newcommand{\compc}[1][\veps]{\mathsf{dec}_{#1}}

\newcommand{\var}{\mathrm{Var}}
\newcommand{\Var}{\var}
\newcommand{\varplus}{\mathrm{Var}_{\sss{+}}}
\newcommand{\Varplus}{\varplus}

\newcommand{\Varm}[1][M]{\Var\sups{#1}}
\newcommand{\Varmbar}[1][\Mbar]{\Var\sups{#1}}


\newcommand{\pmbar}{p_{\sMbar}}
\newcommand{\pmdist}{p\subs{M}}
\newcommand{\PM}{\bbP\sups{M}}
\newcommand{\PMbar}{\bbP\sups{\Mbar}}


\newcommand{\Dbi}[2]{D_{\mathrm{bi}}\prn*{#1\dmid#2}}
\newcommand{\Dbishort}{D_{\mathrm{bi}}}
\newcommand{\cQm}{\cQ_{\cM}}
\newcommand{\cQmh}[1][h]{\cQ_{\cM;#1}}
\newcommand{\cTm}[1][M]{\cT\sups{#1}}
\newcommand{\cTmstar}[1][\Mstar]{\cT\sups{#1}}

\newcommand{\Confone}{R_1}
\newcommand{\Conftwo}{R_2}
\newcommand{\compbi}{\compgen[\mathrm{bi}]}
\newcommand{\compbidual}{\compgendual[\mathrm{bi}]}

\newcommand{\bloss}{\cL}

\newcommand{\cGmbar}{\cG\sups{\Mbar}}
\newcommand{\gmmbar}[1][M]{g\sups{#1;\Mbar}}
\newcommand{\Lbr}{L_{\mathrm{br}}}
\newcommand{\Lbrfull}{L_{\mathrm{br}}(\cM)}
\newcommand{\Lbrfulls}{L^{2}_{\mathrm{br}}(\cM)}

\newcommand{\mum}[1][M]{\mu\sups{#1}}
\newcommand{\wm}[1][M]{w\sups{#1}}
\newcommand{\phim}[1][M]{\phi\sups{#1}}

\newcommand{\AlgEsth}[1][h]{\mathrm{\mathbf{Alg}}_{\mathsf{Est};#1}}
\newcommand{\EstHelh}[1][h]{\mathrm{\mathbf{Est}}_{\mathsf{H};#1}}

\newcommand{\thetam}[1][M]{\theta(#1)}
\newcommand{\thetambar}[1][\Mbar]{\theta(#1)}

\newcommand{\Copt}{C_{\mathrm{opt}}}

\newcommand{\Calpha}{C_{\alpha}}

\newcommand{\dimbi}{d_{\mathrm{bi}}}
\newcommand{\Lbi}{L_{\mathrm{bi}}}
\newcommand{\dimbifull}{d_{\mathrm{bi}}(\cM)}
\newcommand{\dimbifulls}[1][2]{d^{#1}_{\mathrm{bi}}(\cM)}
\newcommand{\Lbifull}{L_{\mathrm{bi}}(\cM)}
\newcommand{\Lbifulls}{L^{2}_{\mathrm{bi}}(\cM)}

\newcommand{\piest}{\pi^{\mathrm{est}}}
\newcommand{\piestm}[1][M]{\pi^{\mathrm{est}}_{\sss{#1}}}
\newcommand{\lest}{\ell^{\mathrm{est}}}
\newcommand{\lestm}[1][M]{\ell^{\mathrm{est}}_{\sss{#1}}}

\newcommand{\Piest}{\Pi^{\mathrm{est}}}

\newcommand{\qbar}{\bar{q}}
\newcommand{\qopt}{q^{\mathrm{opt}}}

\newcommand{\pialpha}{\pi^{\alpha}}
\newcommand{\pialpham}[1][M]{\pi^{\alpha}_{\sss{#1}}}



\newcommand{\con}{x}
\newcommand{\Cspace}{\cX}

\newcommand{\cMx}[1][x]{\cM|_{#1}}
\newcommand{\cMhatx}[1][x]{\cMhat|_{#1}}
\newcommand{\cFmx}[1][x]{\cFm|_{#1}}

\newcommand{\cpol}{\mb{\pi}}
\newcommand{\cpolstar}{\cpol^{\star}}
\newcommand{\cpolm}[1][M]{\cpol\subs{#1}}

\newcommand{\RegCDM}{\Reg_{\mathsf{DM}}}
\newcommand{\EstCD}{\mathrm{\mathbf{Est}}_{\mathsf{D}}}


\newcommand{\relu}{\mathsf{relu}}

\newcommand{\sdis}{\mb{\theta}}
\newcommand{\rdis}{\mb{\psi}}

\newcommand{\Deltanot}{\Delta_0}

\newcommand{\Delm}{\Delta\subs{M}}

\newcommand{\Star}{\mathfrak{s}}
\newcommand{\StarCheck}{\check{\Star}}
\newcommand{\StarDim}{\Star}
\newcommand{\Stardim}{\Star}
\newcommand{\El}{\mathfrak{e}}
\newcommand{\ElCheck}{\check{\El}}
\newcommand{\ElDim}{\El}
\newcommand{\Eldim}{\El}


\newcommand{\errm}[1][M]{\mathrm{err}\sups{#1}}

\newcommand{\hardfamily}{$(\alpha,\beta,\delta)$-family\xspace}
\newcommand{\hardu}{u}
\newcommand{\hardv}{v}

\newcommand{\igwshort}{IGW\xspace}
\newcommand{\igwtext}{inverse gap weighting\xspace}
\newcommand{\pcigw}{\textsf{PC-IGW}\xspace}
\newcommand{\pcigwb}{\textsf{PC-IGW.Bilinear}\xspace}
\newcommand{\pcigwtext}{policy cover inverse gap weighting\xspace}

\newcommand{\igwspanner}{\textsf{IGW-Spanner}\xspace}
\newcommand{\igwargmax}{\textsf{IGW-ArgMax}\xspace}

\newcommand{\oracle}{\mathrm{\mathbf{Alg}}_{\mathsf{Plan}}\xspace}

\newcommand{\I}{\mathrm{Err}_{\mathrm{I}}}
\newcommand{\II}{\mathrm{Err}_{\mathrm{II}}}
\newcommand{\III}{\mathrm{Err}_{\mathrm{III}}}


\newcommand{\MinimaxReg}{\mathfrak{M}(\cM,T)}
\newcommand{\MinimaxRegBayes}{\underbar{\mathfrak{M}}(\cM,T)}


\renewcommand{\emptyset}{\varnothing}

\newcommand{\NullObs}{\crl{\emptyset}}

\newcommand{\filt}{\mathscr{F}}
\newcommand{\ffilt}{\mathscr{F}}
\newcommand{\gfilt}{\mathscr{G}}
\newcommand{\hfilt}{\mathscr{H}}

\newcommand{\hist}{\mathcal{H}}

\newcommand{\Asig}{\mathscr{P}}
\newcommand{\Rsig}{\mathscr{R}}
\newcommand{\Osig}{\mathscr{O}}

\newcommand{\borel}{\mathfrak{B}}

\newcommand{\Hspace}{\Omega}
\newcommand{\Hsig}{\filt}

\newcommand{\dom}{\nu}

\newcommand{\dens}{m}
\newcommand{\densm}[1][M]{m^{\sss{#1}}}

\newcommand{\abscont}{V(\cM)}
\newcommand{\abscontp}{V(\cM')}



\newcommand{\Vmbar}{V^{\sMbar}}


\newcommand{\vepsup}{\bar{\veps}}
\newcommand{\vepslow}{\ubar{\veps}}

\newcommand{\vepsg}{\veps_{\gamma}}

\newcommand{\vepsupg}{\bar{\veps}_{\gamma}}
\newcommand{\vepslowg}{\ubar{\veps}_{\gamma}}

\newcommand{\gameval}[1]{\cV_{\gamma}\sups{#1}}

\newcommand{\Framework}{Decision Making with Structured Observations\xspace}
\newcommand{\FrameworkShort}{DMSO\xspace}

\newcommand{\learner}{learner\xspace}

\newcommand{\Cloc}{c_{\ell}}
\newcommand{\Cglobal}{C(\cM)}

\newcommand{\act}{\pi}
\newcommand{\Act}{\Pi}
\newcommand{\ActSpace}{\Pi}
\newcommand{\ActSize}{\abs{\Pi}}
\newcommand{\ActSizeB}{\abs{\cA}}
\newcommand{\ActSizeRL}{\abs{\cA}}
\newcommand{\ActDist}{\Delta(\Act)}
\newcommand{\action}{decision\xspace}
\newcommand{\actions}{decisions\xspace}
\newcommand{\actstar}{\pistar}


\newcommand{\actb}{a}

\newcommand{\StateSize}{\abs{\cS}}

\newcommand{\obs}{o}
\newcommand{\Obs}{\mathcal{\cO}}
\newcommand{\ObsSpace}{\mathcal{\cO}}
\newcommand{\Ospace}{\mathcal{\cO}}

\newcommand{\RewardSpace}{\cR}
\newcommand{\RSpace}{\RewardSpace}
\newcommand{\Rspace}{\RewardSpace}

\newcommand{\Model}{\cM}
\newcommand{\cMhat}{\wh{\cM}}


\newcommand{\compbasic}{\mathsf{dec}}
\newcommand{\comp}[1][\gamma]{\mathsf{dec}_{#1}}
\newcommand{\comprand}[1][\gamma]{\mathsf{dec}^{\mathrm{rnd}}_{#1}}
\newcommand{\compshort}[1][\gamma]{\mathsf{d}_{#1}}

\newcommand{\compt}[1][\gamma]{\wt{\mathsf{dec}}_{#1}}

\newcommand{\compbar}[1][\gamma]{\overline{\mathsf{dec}}_{#1}}
\newcommand{\compb}[1][\gamma]{\underline{\mathsf{dec}}_{#1}}
\newcommand{\compdual}[1][\gamma]{\compb[#1]}
\newcommand{\compbayes}[1][\gamma]{\compb[#1]}

\newcommand{\compKL}{\compgen[\mathrm{KL}]}
\newcommand{\compKLdual}{\compgendual[\mathrm{KL}]}

\newcommand{\compSq}{\compgen[\mathrm{Sq}]}

\newcommand{\compSqdual}{\compgendual[\mathrm{Sq}]}

\newcommand{\compopt}{\comp^{\mathrm{opt}}}
\newcommand{\compoptdual}{\compb^{\mathrm{opt}}}

\newcommand{\compH}{\compgen[\mathrm{H}]}
\newcommand{\compHdual}{\compgendual[\mathrm{H}]}

\newcommand{\complocshort}{\comp^{\mathrm{loc}}}
\newcommand{\comploc}[2][\gamma]{\mathsf{dec}_{#1,#2}}

\newcommand{\compthmone}{\comploc{\vepslowg}(\cM)}
  \newcommand{\compthmtwo}{\comploc{\vepsupg}(\conv(\cM))}

\newcommand{\comptext}{decision-estimation coefficient\xspace}
\newcommand{\Comptext}{Decision-estimation coefficient\xspace}
\newcommand{\CompText}{Decision-Estimation Coefficient\xspace}
\newcommand{\CompAbbrev}{DEC\xspace}
\newcommand{\CompShort}{\CompAbbrev}

\newcommand{\compgen}[1][D]{\comp^{#1}}
\newcommand{\compgendual}[1][D]{\compb^{#1}}
\newcommand{\compd}[1][D]{\comp^{#1}}

\newcommand{\est}{\mathsf{est}}


\newcommand{\M}[1]{^{{\scriptscriptstyle M}}}  %
\newcommand{\sM}{\sss{M}}
\newcommand{\sMbar}{\sss{\Mbar}}
\renewcommand{\ss}[1]{^{{\scriptscriptstyle#1}}} 
\newcommand{\sups}[1]{^{{\scriptscriptstyle#1}}}
\newcommand{\subs}[1]{_{{\scriptscriptstyle#1}}} 
\renewcommand{\sp}[1]{^{{\scriptscriptstyle#1}}}
\renewcommand{\sb}[1]{_{{\scriptscriptstyle#1}}} 
\newcommand{\sss}[1]{{\scriptscriptstyle#1}}

\newcommand{\Ens}[2]{\En^{\sss{#1},#2}}
\newcommand{\Em}[1][M]{\En^{\sss{#1}}}
\newcommand{\Embar}{\En\sups{\Mbar}}
\newcommand{\Enm}[1][M]{\En^{\sss{#1}}}
\newcommand{\Enmbar}[1][\Mbar]{\En^{\sss{#1}}}
\newcommand{\Prs}[1]{\bbP\sups{#1}}
\newcommand{\bbPs}[1]{\bbP\sups{#1}}
\newcommand{\bbPm}[1][M]{\bbP\sups{#1}}
\newcommand{\bbPmbar}[1][\Mbar]{\bbP\sups{#1}}


\newcommand{\fmhat}{f\sups{\Mhat}}

\newcommand{\fm}[1][M]{f\sups{#1}}
\newcommand{\pim}[1][M]{\pi_{\sss{#1}}}
\newcommand{\pimh}[1][h]{\pi_{\sss{M,#1}}}

\newcommand{\gm}{g\sups{M}}

\newcommand{\Mprime}{M'}
\newcommand{\pimprime}{\pi_{\sss{M'}}}

\newcommand{\cFm}{\cF_{\cM}}
\newcommand{\Pim}{\Pi_{\cM}}
\newcommand{\cMf}{\cM_{\cF}}

\newcommand{\fmbar}{f\sups{\Mbar}}
\newcommand{\pimbar}{\pi\subs{\Mbar}}

\newcommand{\fmstar}{f\sups{\Mstar}}
\newcommand{\pimstar}{\pi\subs{\Mstar}}

\newcommand{\fstar}{f^{\star}}
\newcommand{\pistar}{\pi^{\star}}

\newcommand{\pihat}{\wh{\pi}}

\newcommand{\cMloc}[1][\veps]{\cM_{#1}}

\newcommand{\Mbar}{\wb{M}}

\newcommand{\fmi}{f\sups{M_i}}
\newcommand{\pimi}{\pi\subs{M_i}}

\newcommand{\Jm}{J\sups{M}}
\newcommand{\Rm}[1][M]{R\sups{#1}}
\newcommand{\Pm}[1][M]{P\sups{#1}}
\newcommand{\Pmstar}[1][\Mstar]{P\sups{#1}}

\newcommand{\Pmbar}{P\sups{\Mbar}}
\newcommand{\Rmbar}{R\sups{\Mbar}}


\newcommand{\Prm}[2]{\bbP^{\sss{#1},#2}}

\newcommand{\Jmstar}{J\sups{\Mstar}}

\newcommand{\PiNS}{\Pi_{\mathrm{NS}}} %
\newcommand{\PiRNS}{\Pi_{\mathrm{RNS}}} %
\newcommand{\PiNM}{\Pi_{\mathrm{NM}}} %
\newcommand{\PiGen}{\Pi_{\mathrm{RNS}}} %


\newcommand{\Qmistar}[1][i]{Q^{#1,\star}}
\newcommand{\Vmistar}[1][i]{V^{#1,\star}}

\newcommand{\Qmstar}[1][M]{Q^{\sss{#1},\star}}
\newcommand{\Vmstar}[1][M]{V^{\sss{#1},\star}}
\newcommand{\Qmpi}[1][\pi]{Q^{\sss{M},#1}}
\newcommand{\Vmpi}[1][\pi]{V^{\sss{M},#1}}
\newcommand{\Qmbarpi}[1][\pi]{Q^{\sss{M},#1}}
\newcommand{\Vmbarpi}[1][\pi]{V^{\sss{M},#1}}
\newcommand{\Qm}[2]{Q^{\sss{#1},#2}}
\newcommand{\Vm}[2]{V^{\sss{#1},#2}}

\newcommand{\dmpi}[1][\pi]{d^{\sss{M},#1}}
\newcommand{\dmbarpi}[1][\pi]{d^{\sss{\Mbar},#1}}
\newcommand{\dm}[2]{d^{\sss{#1},#2}}
\newcommand{\dbar}{\bar{d}}
\newcommand{\dtil}{\wt{d}}

\newcommand{\Reg}{\mathrm{\mathbf{Reg}}}
\newcommand{\RegBar}{\widebar{\mathrm{\mathbf{Reg}}}}

\newcommand{\Est}{\mathrm{\mathbf{Est}}}
\newcommand{\EstBar}{\widebar{\mathrm{\mathbf{Est}}}}

\newcommand{\EstHel}{\mathrm{\mathbf{Est}}_{\mathsf{H}}}
\newcommand{\EstOnHel}{\mathrm{\mathbf{Est}}^{\mathsf{on}}_{\mathsf{H}}}
\newcommand{\EstBarHel}{\widebar{\mathrm{\mathbf{Est}}}_{\mathsf{H}}}
\newcommand{\EstProbHel}{\mathrm{\mathbf{Est}}_{\mathsf{H}}(T,\delta)}
\newcommand{\EstH}{\EstHel}

\newcommand{\EstD}{\mathrm{\mathbf{Est}}_{\mathsf{D}}}

\newcommand{\EstSq}{\mathrm{\mathbf{Est}}_{\mathsf{Sq}}}

\newcommand{\EstKL}{\mathrm{\mathbf{Est}}_{\mathsf{KL}}}

\newcommand{\RegDM}{\Reg_{\mathsf{DM}}}
\newcommand{\RegBarDM}{\RegBar_{\mathsf{DM}}}

\newcommand{\RegB}{\RegBandit}
\newcommand{\RegMAB}{\RegBandit}
  \newcommand{\RegBarMAB}{\RegBar_{\mathsf{B}}}
  \newcommand{\RegBandit}{\mathrm{\mathbf{Reg}}_{\mathsf{B}}}

  \newcommand{\RegRL}{\Reg_{\mathsf{RL}}}
\newcommand{\RegBarRL}{\RegBar_{\mathsf{RL}}}


\newcommand{\RegOL}{\mathrm{\mathbf{Reg}}_{\mathsf{OL}}(T,\delta)}
  \newcommand{\AlgOL}{\mathrm{\mathbf{Alg}}_{\mathsf{OL}}}
  \newcommand{\RegOLShort}{\Reg_{\mathsf{OL}}}
  
  \newcommand{\RegBR}{\Reg_{\mathsf{BR}}}
  \newcommand{\RegSB}{\Reg_{\mathsf{SB}}}
  \newcommand{\RegSquare}{\Reg_{\mathsf{Sq}}}
  
  \newcommand{\RegCB}{\mathrm{\mathbf{Reg}}_{\mathsf{CB}}}
  \newcommand{\RegBarCB}{\widebar{\mathrm{\mathbf{Reg}}}_{\mathsf{CB}}}


  
  \newcommand{\AlgEst}{\mathrm{\mathbf{Alg}}_{\mathsf{Est}}}

  \newcommand{\logloss}{\ls_{\mathrm{\log}}}

  \newcommand{\RegLog}{\Reg_{\mathsf{KL}}}
  \newcommand{\RegBarLog}{\widebar{\Reg}_{\mathsf{KL}}}
    \newcommand{\RegLogT}{\Reg_{\mathsf{KL}}(T)}


    \newcommand{\MComp}{\mathsf{est}(\cM,T)}
    \newcommand{\Mcomp}{\mathsf{est}(\cM,T)}
    
    \newcommand{\GComp}{\mathsf{est}(\cG,T)}
    \newcommand{\Gcomp}{\mathsf{est}(\cG,T)}

    \newcommand{\QComp}{\mathsf{est}(\cQm,T)}
    \newcommand{\Qcomp}{\mathsf{est}(\cQm,T)}
    
    \newcommand{\PComp}{\mathsf{est}(\cP,T)}
    \newcommand{\PComph}[1][h]{\mathsf{est}(\cP_{#1},T)}
    
    \newcommand{\ActComp}{\mathsf{est}(\Pim,T)}
    \newcommand{\AComp}{\mathsf{est}(\Pim,T)}
    \newcommand{\Acomp}{\mathsf{est}(\Pim,T)}

\newcommand{\MCov}[1][\veps]{\cN(\cM,#1)}
    \newcommand{\ActCov}[1][\veps]{\cN(\Pim,#1)}
    

  \newcommand{\mathrmb}[1]{\mathrm{\mathbf{#1}}}

\newcommand{\Mhat}{\wh{M}}
\newcommand{\Mstar}{M^{\star}}

  \newcommand{\bbPl}{\bbP_{\lambda}}
  \newcommand{\bbQl}{\bbQ_{\lambda}}

\newcommand{\cAhat}{\wh{\cA}}

  \newcommand{\ghat}{\wh{g}}

\newcommand{\thetahat}{\wh{\theta}}
\newcommand{\thetastar}{\theta^{\star}}

\newcommand{\tens}{\otimes}

\newcommand{\Rbar}{\wb{R}}

\newcommand{\Pbar}{\widebar{P}}

\newcommand{\starucb}{star hull UCB\xspace}
\newcommand{\starucblong}{star hull upper confidence bound\xspace}

\newcommand{\optionone}{\textsc{Option I}\xspace}
\newcommand{\optiontwo}{\textsc{Option II}\xspace}


\newcommand{\Dis}{\mathrm{Dis}}

\newcommand{\xdist}{\cD}
\newcommand{\rdist}{\bbP_{r}}

\newcommand{\algcomment}[1]{\textcolor{blue!70!black}{\small{\texttt{\textbf{//\hspace{2pt}#1}}}}}
\newcommand{\algcommentlight}[1]{\textcolor{blue!70!black}{\transparent{0.5}\small{\texttt{\textbf{//\hspace{2pt}#1}}}}}
\newcommand{\algcommentbig}[1]{\textcolor{blue!70!black}{\footnotesize{\texttt{\textbf{/*
          #1~*/}}}}}
\newcommand{\algcolor}[1]{\textcolor{blue!70!black}{#1}}
\newcommand{\algspace}{\hspace{\algorithmicindent}}


\newcommand{\Holder}{H{\"o}lder\xspace}

\newcommand{\Otilde}{\wt{O}}

\newcommand{\midsem}{\,;}

\newcommand{\trn}{\top}
\newcommand{\pinv}{\dagger}
\newcommand{\psdleq}{\preceq}
\newcommand{\psdgeq}{\succeq}
\newcommand{\psdlt}{\prec}
\newcommand{\psdgt}{\succ}
\newcommand{\approxleq}{\lesssim}
\newcommand{\approxgeq}{\gtrsim}

\newcommand{\opnorm}{\mathsf{op}}

\newcommand{\eigmin}{\lambda_{\mathrm{min}}}
\newcommand{\eigmax}{\lambda_{\mathrm{max}}}

\renewcommand{\tC}{\tilde{\cC}}

\newcommand{\zero}{\mathbf{0}}

\newcommand{\Id}{I}

\newcommand{\bq}{\mathbf{q}}

\newcommand{\xpi}{x^{\pi}}
\newcommand{\phipi}{\phi^{\pi}}

\newcommand{\lw}{\bar{w}}

\newcommand{\bu}{\mb{u}}
\newcommand{\bv}{\mb{v}}
\newcommand{\bz}{\mb{z}}
\newcommand{\bw}{\mb{w}}

\newcommand{\xt}{x_t}
\newcommand{\xto}{x_{t+1}}

\newcommand{\expone}{(1)}
\newcommand{\exptwo}{(2)}

\newcommand{\xl}[1][T]{x_{1:#1}}
\newcommand{\xr}[1][t]{x_{#1:T}}
\newcommand{\ul}[1][T]{u_{1:#1}}
\newcommand{\ur}[1][t]{u_{#1:T}}
\newcommand{\wl}[1][T]{w_{1:#1}}
\renewcommand{\wr}[1][t]{w_{#1:T}}

\newcommand{\fhat}{\wh{f}}
\newcommand{\ahat}{\wh{a}}
\newcommand{\fbar}{\bar{f}}

\renewcommand{\ind}[1]{^{{\scriptscriptstyle#1}}}

\newcommand{\xh}{x_h}
\newcommand{\rh}{r_h}
\renewcommand{\rh}{r_h}
\newcommand{\xhp}{x_{h+1}}



\newcommand{\bigoh}{O}
\newcommand{\bigoht}{\wt{O}}
\newcommand{\bigom}{\Omega}
\newcommand{\bigomt}{\wt{\Omega}}
\newcommand{\bigthetat}{\wt{\Theta}}

\newcommand{\indic}{\mathbb{I}}




\newcommand{\overleq}[1]{\overset{#1}{\leq{}}}
\newcommand{\overgeq}[1]{\overset{#1}{\geq{}}}
\newcommand{\overlt}[1]{\overset{#1}{<}}
\newcommand{\overgt}[1]{\overset{#1}{>}}
\newcommand{\overeq}[1]{\overset{#1}{=}}

\renewcommand{\Pr}{\bbP}

\newcommand{\ftilde}{\tilde{f}}
\newcommand{\fcheck}{\check{f}}
\newcommand{\gtilde}{\tilde{g}}
\newcommand{\empcov}{\wh{\cF}}
\newcommand{\Sbad}{S_{\mathrm{bad}}}
\newcommand{\aprime}{a'}

\newcommand{\undertext}[2]{\underbrace{#1}_{\text{#2}}}

\newcommand{\fup}{\bar{f}}
\newcommand{\flow}{\underbar{f}}

\newcommand{\aone}{a\ind{1}}
\newcommand{\atwo}{a\ind{2}}

\newcommand{\cb}{\mathsf{A}}

\newcommand{\poly}{\mathrm{poly}}
\newcommand{\polylog}{\mathrm{polylog}}


\newcommand{\Dsq}[2]{D_{\mathsf{Sq}}\prn*{#1,#2}}
\newcommand{\Dsqshort}{D_{\mathsf{Sq}}}

\newcommand{\kl}[2]{D_{\mathsf{KL}}\prn*{#1\,\|\,#2}}
\newcommand{\Dkl}[2]{D_{\mathsf{KL}}\prn*{#1\,\|\,#2}}
\newcommand{\Dklshort}{D_{\mathsf{KL}}}
\newcommand{\Dhel}[2]{D_{\mathsf{H}}\prn*{#1,#2}}
\newcommand{\Dgen}[2]{D\prn*{#1\dmid{}#2}}
\newcommand{\Dgent}[2]{D\ind{t}\prn*{#1\dmid{}#2}}
\newcommand{\Dhels}[2]{D^{2}_{\mathsf{H}}\prn*{#1,#2}}
\newcommand{\Ddel}[2]{D_{\Delta}\prn*{#1,#2}}
\newcommand{\Dhelshort}{D^{2}_{\mathsf{H}}}
\newcommand{\Dchis}[2]{D_{\chi^2}\prn*{#1\dmid{}#2}}
\newcommand{\DchisX}[3]{D_{\chi^2}\prn[#1]{#2\dmid{}#3}}
\newcommand{\Dtris}[2]{D^{2}_{\Delta}\prn*{#1,#2}}
\newcommand{\Dtri}[2]{D_{\Delta}\prn*{#1,#2}}
\newcommand{\Dtv}[2]{D_{\mathsf{TV}}\prn*{#1,#2}}
\newcommand{\Dtvs}[2]{D^2_{\mathsf{TV}}\prn*{#1,#2}}
\newcommand{\dkl}[2]{d_{\mathsf{KL}}\prn*{#1\,\|\,#2}}
\newcommand{\Dphi}[2]{D_{\phi}(#1\;\|\;#2)}
\newcommand{\dphi}[2]{d_{\phi}(#1\;\|\;#2)}
\newcommand{\klr}[2]{D_{\mathsf{re}}(#1\;\|\;#2)}
\newcommand{\tv}[2]{D_{\mathsf{tv}}(#1\;\|\;#2)}

\newcommand{\DhelsX}[3]{D^{2}_{\mathsf{H}}\prn[#1]{#2,#3}}

\newcommand{\Ber}{\mathrm{Ber}}
\newcommand{\Rad}{\mathrm{Rad}}
\newcommand{\dmid}{\;\|\;}

\newcommand{\conv}{\mathrm{co}}
\newcommand{\diam}{\mathrm{diam}}


\newcommand{\bls}{\mb{\ls}}

\newcommand{\brak}{{\tiny[]}}

\newcommand{\Deltagap}{\Delta_{\mathrm{policy}}}
\newcommand{\Picsc}{\Pi^{\mathrm{csc}}}

\newcommand{\vcdim}{\mathrm{vcdim}}

\newcommand{\adacb}{\textsf{AdaCB}\xspace}
\newcommand{\squarecb}{\textsf{SquareCB}\xspace}
\newcommand{\falcon}{\textsf{FALCON}\xspace}


\newcommand{\Vf}{V}
\newcommand{\Qf}{Q}

\newcommand{\Qhat}{\wh{\Qf}}
\newcommand{\Vhat}{\wh{\Vf}}

\newcommand{\Vpi}{\Vf^{\pi}}
\newcommand{\Qpi}{\Qf^{\pi}}

\newcommand{\rmax}{\textsf{Rmax}\xspace}
\newcommand{\valueiteration}{\textsf{ValueIteration}\xspace}

\newcommand{\labelme}[1]{\tag{\theequation}\label{#1}}

\newcommand{\Ssafe}{\cS_{\mathrm{safe}}}
\newcommand{\Esafe}{\cE_{\mathrm{safe}}}
\newcommand{\Tsafe}{T_{\mathrm{safe}}}
\newcommand{\unif}{\mathrm{unif}}

\newcommand{\starhull}{\mathrm{star}}

\newcommand{\pescape}{P_{\mathrm{escape}}}
\newcommand{\vepsucb}{\veps_{\mathrm{ucb}}}
\newcommand{\vepsstati}{\veps_{\mathrm{stat,I}}}
\newcommand{\vepsstatii}{\veps_{\mathrm{stat,II}}}
\newcommand{\nstat}{n_{\mathrm{stat}}}
\newcommand{\Phat}{\wh{P}}

\newcommand{\Ffilt}{\mathfrak{F}}
\newcommand{\Eescape}{\cE_{\textrm{escape}}}

\newcommand{\vepshat}{\wh{\veps}}
\newcommand{\vepsbar}{\widebar{\veps}}
\newcommand{\igw}{\textsf{IGW}}
\newcommand{\ssep}{;\,}
\newcommand{\sh}[1][h]{s_{#1}}

\newcommand{\qh}{q_h}
\newcommand{\Qh}{Q_h}
\newcommand{\im}{\ind{m}}
\newcommand{\sep}{\ssep}
\newcommand{\Creg}{C_{\mathrm{reg}}}
\newcommand{\creg}{c_{\mathrm{reg}}}
\newcommand{\Cucb}{C_{\mathrm{ucb}}}
\newcommand{\gammam}{\gamma\im}

\newcommand{\Eopt}{\cE_{\mathrm{opt}}}

\newcommand{\emi}{\psi}
\newcommand{\dirsum}{\oplus}
\newcommand{\piunif}{\pi_{\mathrm{unif}}}
\newcommand{\cPhat}{\wh{\cP}}

\newcommand{\supp}{\mathrm{supp}}

\newcommand{\cPbar}{\wb{\cP}}


\newcommand{\Pstar}{P^{\star}}
\newcommand{\Plbar}{\underbar{P}}
\newcommand{\Ptil}{\wt{P}}
\newcommand{\astar}{a^{\star}}

\newcommand{\cFhat}{\wh{\cF}}
\newcommand{\cFbar}{\widebar{\cF}}
\newcommand{\Vtil}{\wt{\Vf}}
\newcommand{\Qtil}{\wt{\Qf}}
\newcommand{\ftil}{\tilde{f}}

\newcommand{\mathand}{\quad\text{and}\quad}
\newcommand{\mathwhere}{\quad\text{where}\quad}


\def\multiset#1#2{\ensuremath{\left(\kern-.3em\left(\genfrac{}{}{0pt}{}{#1}{#2}\right)\kern-.3em\right)}}


\newcommand{\grad}{\nabla}
\newcommand{\diag}{\mathrm{diag}}

\newcommand{\op}{\mathrm{op}}

\newcommand{\iid}{i.i.d.\xspace}

\renewcommand{\ls}{\ell}


\newcommand{\glcomp}{c}

\newcommand{\InfB}{\mathcal{I}_{\mathrm{B}}}
\newcommand{\InfF}{\mathcal{I}_{\mathrm{F}}}

\renewcommand{\emptyset}{\varnothing}

\newcommand{\what}{\wh{w}}


\newcommand{\pbar}{\bar{p}}
\newcommand{\phat}{\wh{p}}

\newcommand{\Meps}{M_{\veps}}

\newcommand{\MA}{\mathcal{A}}
\newcommand{\norm}[1]{\left \lVert #1 \right \rVert}
\DeclareMathOperator*{\EE}{\mathbb{E}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\st}{\star}
\newcommand{\BP}{\mathbb{P}}
\newcommand{\BQ}{\mathbb{Q}}
\newcommand{\NP}{\mathsf{NP}}
\newcommand{\RP}{\mathsf{RP}}
\newcommand{\Alg}{\mathtt{Alg}}
\newcommand{\MX}{\mathcal{X}}
\newcommand{\MO}{\mathcal{O}}
\newcommand{\MP}{\mathcal{P}}
\newcommand{\MD}{\mathcal{D}}
\DeclareMathOperator{\Bin}{Bin}
\newcommand{\LPN}{\mathsf{LPN}}
\DeclareMathOperator*{\Prr}{Pr}
\DeclareMathOperator{\Law}{Law}
\DeclareMathOperator{\Maj}{\mathsf{MAJ}}
\newcommand{\phiver}{\phi^{\mathsf{ver}}}
\newcommand{\Ofeat}{\mathcal{O}_{\mathsf{feat}}}
\newcommand{\Osamp}{\mathcal{O}_{\mathsf{samp}}}
\newcommand{\Cmis}{C_{\mathsf{mis}}}
\newcommand{\ME}{\mathcal{E}}
\newcommand{\xtest}{x^{\mathsf{test}}}
\newcommand{\ytest}{y^{\mathsf{test}}}
\newcommand{\Adv}{\mathtt{Adv}}
\newcommand{\LL}{\mathcal{L}}
\newcommand{\taulin}{\tau_{\mathsf{lin}}}
\newcommand{\epapx}{\varepsilon_{\mathsf{apx}}}
\newcommand{\mol}[2]{\mathsf{mol}_{#1}(#2)}
\newcommand{\epstat}{\varepsilon_{\mathsf{stat}}}
\newcommand{\MS}{\mathcal{S}}
\newcommand{\MF}{\mathcal{F}}
\newcommand{\MG}{\mathcal{G}}
\newcommand{\uop}[2]{\mathbf{u}(#1,#2)}
\newcommand{\emploss}{\mathcal{\wh L}}
\newcommand{\epopt}{\varepsilon_{\mathsf{opt}}}
\newcommand{\MT}{\mathcal{T}}
\newcommand{\Cond}[2]{\mathsf{Cond}_{#1}[#2]}
\newcommand{\kfake}{k^{\mathsf{fake}}}
\newcommand{\bfo}{\mathbf{1}}
\newcommand{\bfz}{\mathbf{0}}
\newcommand{\Ovec}{\mathcal{O}_{\mathsf{vec}}}
\newcommand{\Oproj}{\mathcal{O}_{\mathsf{proj}}}
\newcommand{\epproj}{\varepsilon_{\mathsf{proj}}}
\newcommand{\PGD}{\mathtt{PGD}}
\newcommand{\MY}{\mathcal{Y}}
\newcommand{\alphatil}{\widetilde\alpha}
\newcommand{\betatil}{\widetilde\beta}
\newcommand{\KernRho}{\mathtt{KernelizedRho}}
\DeclareMathOperator{\Proj}{Proj}
\DeclareMathOperator{\vspan}{span}
\newcommand{\MB}{\mathcal{B}}
\newcommand{\Jeps}{\wh J_\epsilon}
\newcommand{\Keps}{\wh K_\epsilon}
\newcommand{\Veps}{\wh V_\epsilon}
\newcommand{\Weps}{\wh W_\epsilon}
\newcommand{\Jlarge}{\wh J_{\mathsf{large}}}
\newcommand{\Klarge}{\wh K_{\mathsf{large}}}
\newcommand{\Blarge}{B_{\mathsf{large}}}
\newcommand{\Vlarge}{\wh V_{\mathsf{large}}}
\newcommand{\ChunkKR}{\mathtt{ChunkKR}}




==> section_lower.tex <==

\begin{theorem}
\end{theorem}

\begin{theorem}\label{thm:lower}
    For any $\vepsrm \in (0, 1/4]$, there exists a problem instance and comparator policy $\pistar$ 
    with $\Cone[\pistar]=\bigoht(1)$
    such that if $N =\bigoht(\vepsrm^{-1})$ 
    then  
    \begin{align}
       J(\pistar) - J(\pi_{\cA}) = \wt\Omega\rbr*{\vepsrm^{-1}},
    \end{align}
    where $\pi_{\cA}$ is the policy induced by any selection strategy $\cA$.

\end{theorem}




==> section_scratch.tex <==
%

%



==> widebar.tex <==

\makeatletter
\let\save@mathaccent\mathaccent
\newcommand*\if@single[3]{%
  \setbox0\hbox{${\mathaccent"0362{#1}}^H$}%
  \setbox2\hbox{${\mathaccent"0362{\kern0pt#1}}^H$}%
  \ifdim\ht0=\ht2 #3\else #2\fi
  }
\newcommand*\rel@kern[1]{\kern#1\dimexpr\macc@kerna}
\newcommand*\widebar[1]{\@ifnextchar^{{\wide@bar{#1}{0}}}{\wide@bar{#1}{1}}}
\newcommand*\underbar[1]{\@ifnextchar_{{\under@bar{#1}{0}}}{\under@bar{#1}{1}}}
\newcommand*\wide@bar[2]{\if@single{#1}{\wide@bar@{#1}{#2}{1}}{\wide@bar@{#1}{#2}{2}}}
\newcommand*\under@bar[2]{\if@single{#1}{\under@bar@{#1}{#2}{1}}{\under@bar@{#1}{#2}{2}}}
\newcommand*\wide@bar@[3]{%
  \begingroup
  \def\mathaccent##1##2{%
    \let\mathaccent\save@mathaccent
    \if#32 \let\macc@nucleus\first@char \fi
    \setbox\z@\hbox{$\macc@style{\macc@nucleus}_{}$}%
    \setbox\tw@\hbox{$\macc@style{\macc@nucleus}{}_{}$}%
    \dimen@\wd\tw@
    \advance\dimen@-\wd\z@
    \divide\dimen@ 3
    \@tempdima\wd\tw@
    \advance\@tempdima-\scriptspace
    \divide\@tempdima 10
    \advance\dimen@-\@tempdima
    \ifdim\dimen@>\z@ \dimen@0pt\fi
    \rel@kern{0.6}\kern-\dimen@
    \if#31
      \overline{\rel@kern{-0.6}\kern\dimen@\macc@nucleus\rel@kern{0.4}\kern\dimen@}%
      \advance\dimen@0.4\dimexpr\macc@kerna
      \let\final@kern#2%
      \ifdim\dimen@<\z@ \let\final@kern1\fi
      \if\final@kern1 \kern-\dimen@\fi
    \else
      \overline{\rel@kern{-0.6}\kern\dimen@#1}%
    \fi
  }%
  \macc@depth\@ne
  \let\math@bgroup\@empty \let\math@egroup\macc@set@skewchar
  \mathsurround\z@ \frozen@everymath{\mathgroup\macc@group\relax}%
  \macc@set@skewchar\relax
  \let\mathaccentV\macc@nested@a
  \if#31
    \macc@nested@a\relax111{#1}%
  \else
    \def\gobble@till@marker##1\endmarker{}%
    \futurelet\first@char\gobble@till@marker#1\endmarker
    \ifcat\noexpand\first@char A\else
      \def\first@char{}%
    \fi
    \macc@nested@a\relax111{\first@char}%
  \fi
  \endgroup
}
\newcommand*\under@bar@[3]{%
  \begingroup
  \def\mathaccent##1##2{%
    \let\mathaccent\save@mathaccent
    \if#32 \let\macc@nucleus\first@char \fi
    \setbox\z@\hbox{$\macc@style{\macc@nucleus}_{}$}%
    \setbox\tw@\hbox{$\macc@style{\macc@nucleus}{}_{}$}%
    \dimen@\wd\tw@
    \advance\dimen@-\wd\z@
    \divide\dimen@ 3
    \@tempdima\wd\tw@
    \advance\@tempdima-\scriptspace
    \divide\@tempdima 10
    \advance\dimen@-\@tempdima
    \ifdim\dimen@>\z@ \dimen@0pt\fi
    \rel@kern{0.6}\kern-\dimen@
    \if#31
      \underline{\rel@kern{-0.6}\kern\dimen@\macc@nucleus\rel@kern{0.4}\kern\dimen@}%
      \advance\dimen@0.4\dimexpr\macc@kerna
      \let\final@kern#2%
      \ifdim\dimen@<\z@ \let\final@kern1\fi
      \if\final@kern1 \kern-\dimen@\fi
    \else
      \underline{\rel@kern{-0.6}\kern\dimen@#1}%
    \fi
  }%
  \macc@depth\@ne
  \let\math@bgroup\@empty \let\math@egroup\macc@set@skewchar
  \mathsurround\z@ \frozen@everymath{\mathgroup\macc@group\relax}%
  \macc@set@skewchar\relax
  \let\mathaccentV\macc@nested@a
  \if#31
    \macc@nested@a\relax111{#1}%
  \else
    \def\gobble@till@marker##1\endmarker{}%
    \futurelet\first@char\gobble@till@marker#1\endmarker
    \ifcat\noexpand\first@char A\else
      \def\first@char{}%
    \fi
    \macc@nested@a\relax111{\first@char}%
  \fi
  \endgroup
}
\makeatother


